FedQPL: A Language for Logical Query Plans over Heterogeneous Federations of RDF Data Sources (Extended Version)

Federations of RDF data sources provide great potential when queried for answers and insights that cannot be obtained from one data source alone. A challenge for planning the execution of queries over such a federation is that the federation may be heterogeneous in terms of the types of data access interfaces provided by the federation members. This challenge has not received much attention in the literature. This paper provides a solid formal foundation for future approaches that aim to address this challenge. Our main conceptual contribution is a formal language for representing query execution plans; additionally, we identify a fragment of this language that can be used to capture the result of selecting relevant data sources for different parts of a given query. As technical contributions, we show that this fragment is more expressive than what is supported by existing source selection approaches, which effectively highlights an inherent limitation of these approaches. Moreover, we show that the source selection problem is NP-hard and in $\Sigma_2^\mathrm{P}$, and we provide a comprehensive set of rewriting rules that can be used as a basis for query optimization.

==> algebra.tex <==
\section{Logical Query Plans} \label{sec:QueryPlans}

The next query planning step after source selection is to create and optimize a logical query plan. Such a plan is typically a tree of algebraic operators that capture a declarative notion of how their output is related to their input~(rather than a concrete algorithm of how the output will be produced). The logical plan also indicates an order in which the operators will be evaluated.

We observe that in  the literature on query engines for~(homogeneous) federations of RDF data such plans are treated very informally. That is, the authors talk about such plans only in terms of \hidden{a few }examples, where these examples are typically informal illustrations that visually represent some form of a tree in which the leaf nodes are one or more triple patterns with various annotations and the internal nodes are operators from the SPARQL algebra~(sometimes in combination with some additional, in\-for\-mal\-ly-in\-tro\-duced operators~\cite{schwarte2011fedx}).

In this section we introduce an algebra
	%\removable{that can be used as a language}
to describe such logical query plans formally. This
	algebra, which we call \emph{HetFedA},
	%language
can be applied both to define query planning and optimization approaches in a more precise
	%\removable{and less ambiguous}
manner and to actually represent the logical plans in a query engine. The algebra features operators to explicitly capture the intention to execute a particular subquery at a specific federation member and to
	%\removable{explicitly}
distinguish whether such an access to a federation member is meant to be based solely on the given subquery or also on intermediate results obtained for other subqueries.
	%While these features can be leveraged by approaches that focus on homogeneous federations, we argue that they
	We argue that such features
are paramount for any principled approach to query planning in heterogeneous federations where
	the characteristics and limitations of different
	%the differences of
	%different
data access interfaces have to be taken into account%
	\removable{~(and, certainly, these features can also be leveraged when defining new approaches that focus on homogeneous federations)}%
.

In the following, we first define the operators of our algebra and show how they can be combined into an initial logical query plan, and thereafter we introduce rewriting rules that can be used for logical query optimization.


	%\subsection{Algebra}
	\subsection{HetFedA Operators and Expressions}
\label{ssec:Algebra}

Our first operator---which is, in fact, a family of operators for all types of interfaces---captures the
	%\removable{intention} to retrieve
	retrieval of
the result of a given (sub)query from a given federation member, where this
	%federation
member
	%provides
	has
the corresponding type of interface and the (sub)query
	can be
	%is
expressed in the request language of that~interface.

\begin{mydefinition} \label{def:request}
For every interface~$\iface = \ifaceTuple$, let $\ifaceReqLangExp$ be an expression in~$\ifaceReqLang{}$ and let $\member = (\symRDFgraph,\iface)$ be a federation member~(with interface~$\iface)$;
the \definedTerm{$\iface$-spe\-cif\-ic request result} for $\ifaceReqLangExp$ over~$\member$, denoted by $\request{\ifaceReqLangExp}{\member}$, is
	a set of solution mappings that is defined as \removable{follows:}
	%a set of solution mappings that is defined as
	%the following set of solution mappings:
$\request{\ifaceReqLangExp}{\member} \definedAs \omega\bigl( \ifaceFct(\ifaceReqLangExp,\symRDFgraph) \bigr)$.
\end{mydefinition}

\begin{myexample} \label{ex:request}
Recall the source assignment~$a'_\mathsf{ex}$ in Example~\ref{ex:SourceAssignment:Syntax}.
	%The
	Its
access to federation members $\member_1$, $\member_2$, and $\member_3$
	%in $a'_\mathsf{ex}$
can be represented \removable{in a logical plan} by the operators $\request{\symTP_1}{\member_1\!}$, $\request{\symTP_2}{\member_2\!}$, and $\request{\lbrace\symTP_1,\symTP_2\rbrace\!}{\member_3}$, respectively. Notice that the latter of these requests is possible only because the interface of $\member_3$ is the SPARQL endpoint interface~$\iface_\mathsf{sparql}$~(cf.\ Example~\ref{ex:Federation}); e.g., with $\iface_\mathsf{TPF}$ it would not be possible.
\end{myexample}

The second
	%operator~(more precisely, family of operators for all triple pattern accessible interfaces)
	family of operators~(for all triple pattern accessible interfaces)
	%operator
captures the intention to access a\hidden{~(triple pattern accessible)} federation member to obtain solution mappings for a single triple pattern that need to be compatible with (and are to be joined with) solution mappings in a given intermediate query result.
 
\begin{mydefinition} \label{def:tpAdd}
For every interface~$\iface = \ifaceTuple$ that supports triple pattern requests, let $\member = (\symRDFgraph,\iface)$ be a federation member~(with interface~$\iface)$,
	%\removable{let}
$\symTP$~be a triple pattern, and $\Omega$~be a set of solution mappings;
the \definedTerm{$\iface$-spe\-cif\-ic triple pattern result addition} to~$\Omega$ for $\symTP$ over~$\member$, denoted by $\tpAdd{\Omega}{\symTP}{\member}$, is
	%a set of solution mappings that is defined as \removable{follows:}
	a set of solution mappings that is defined as:
	%the following set of solution mappings:
$\tpAdd{\Omega}{\symTP}{\member} \definedAs \Omega \Join \omega\bigl( \ifaceFct(\symTP,\symRDFgraph) \bigr)$.
\end{mydefinition}

\begin{myexample} \label{ex:tpAdd}
The subexpression
$\saJL
	\saBL \lbrace \symTP_1 \rbrace \saBM \member_1 \saBR \otimes \saBL\lbrace \symTP_2 \rbrace \saBM \member_2 \saBR
\saJR$ of source assignment~$a'_\mathsf{ex}$ in Example~\ref{ex:SourceAssignment:Syntax} may be represented
	%\removable{in a logical plan}
by
	%combining a $\xxxAlgebraOperatorName{req}$ operator with a following $\xxxAlgebraOperatorName{tpAdd}$ operator
	%putting a $\xxxAlgebraOperatorName{tpAdd}$ operator on top of a $\xxxAlgebraOperatorName{req}$ operator%
	%a $\xxxAlgebraOperatorName{tpAdd}$ operator that has a $\xxxAlgebraOperatorName{req}$ operator as input%
	a $\xxxAlgebraOperatorName{tpAdd}$ operator with a $\xxxAlgebraOperatorName{req}$ operator as input%
, which gives us
	\removable{either}
$\tpAddB{ \request{\symTP_2}{\member_2\!} }{\symTP_1}{\member_1\!}$ or $\tpAddB{ \request{\symTP_1}{\member_1\!} }{\symTP_2}{\member_2\!}$.
\end{myexample}

We
	%emphasize that the $\xxxAlgebraOperatorName{tpAdd}$ operator can be used
	may use the $\xxxAlgebraOperatorName{tpAdd}$ operator
in cases in which the processing power of a federation member can be exploited to produce the join between an input set of solution mappings and the result of evaluating a triple pattern over the data of that federation member. Specific algorithms
	%(physical operators)
that can be used as implementations of $\xxxAlgebraOperatorName{tpAdd}$ in such cases are RDF-specific variations of the semijoin~\cite{DBLP:journals/tods/BernsteinGWRR81} and the bind join~\cite{DBLP:conf/vldb/HaasKWY97}. Concrete examples of such algorithms
	%are Zemanek et al.'s distributed semi-join~\cite{zemanek2008optimizing}, G{\"{o}}rlitz and Staab's semi join and bind join~\cite{DBLP:series/sci/GorlitzS11,gorlitz2011splendid}, Schwarte et al.'s bound join~\cite{schwarte2011fedx}, Charalambidis et al.'s bind join~\cite{charalambidis2015semagrow}, Saleem et al.'s bind join~\cite{saleem2018costfed}, and Hartig and Buil-Aranda's brTPF client algorithm~\cite{hartig2016brtpf}.
	can be found in the SPARQL endpoint federation engines FedX~\cite{schwarte2011fedx}, \hidden{SPLENDID~\cite{gorlitz2011splendid}, }SemaGrow~\cite{charalambidis2015semagrow}, and CostFed~\cite{saleem2018costfed}, as well as in the brTPF client~\cite{hartig2016brtpf}.
Such algorithms rely on a data access interface in which the given input solution mappings can be captured as part of the requests.
However,
	for less expressive interfaces~(such as the TPF interface),
the $\xxxAlgebraOperatorName{tpAdd}$ operator can also be implemented using
	%some form of distributed index nested-loops join
	a variation of an index nested-loops join
in which
	a separate request is created for each input solution mapping%
	%each input solution mapping is applied to the given triple pattern and then send as a separate request%
~%
	%\cite{quilitz2008querying,vidal2010efficiently,verborgh2016triple}.
	%\cite{quilitz2008querying,verborgh2016triple}.
	\cite{verborgh2016triple}.

\removable{
\begin{myexample} \label{ex:tpAdd-2}
Recall the two
	\removable{possible}
options in
	\removable{the previous example~(}Example~\ref{ex:tpAdd}),
	%Example~\ref{ex:tpAdd},
$\tpAddB{ \request{\symTP_2}{\member_2\!} }{\symTP_1}{\member_1\!}$ and $\tpAddB{ \request{\symTP_1}{\member_1\!} }{\symTP_2}{\member_2\!}$.
Considering that the interface of federation member~$\member_1$ is
	a brTPF interface
	%$\iface_\mathsf{brTPF}$
whereas $\member_2$ has a TPF interface~(cf.\ Example~\ref{ex:Federation}), we may prefer the first
	%of the two options in Example~\ref{ex:tpAdd}
	option
because it 
	%provides for a greater number of algorithms to choose from during
	opens more choices for
physical query optimization~(e.g., implementing $\xxxAlgebraOperatorName{tpAdd}$ over
	%a brTPF interface may be done by using a bind join algorithm~\cite{hartig2016brtpf}, which is not the case for a TPF interface).
	brTPF may be done by using a bind join algorithm~\cite{hartig2016brtpf}, which is impossible with TPF).
	%brTPF may be done by using a bind join algorithm~\cite{hartig2016brtpf}, which is not the case for TPF).
On the other hand, a query optimizer may estimate a significantly smaller result size for $\request{\symTP_1}{\member_1\!}$ than for $\request{\symTP_2}{\member_2\!}$, which could justify choosing the second~option.
\end{myexample}
}

The next family of operators represents a BGP-based
	counterpart
	%variation
of
	%the \removable{previous} operator.
	%the $\xxxAlgebraOperatorName{tpAdd}$ \removable{operator}.
	$\xxxAlgebraOperatorName{tpAdd}$.

\begin{mydefinition} \label{def:bgpAdd}
For every interface~$\iface = \ifaceTuple$ that supports BGP requests, let $\member = (\symRDFgraph,\iface)$ be a federation member~(with interface~$\iface)$,
	%\removable{let}
$\symBGP$~be a BGP, and $\Omega$~be a set of solution mappings;
the \definedTerm{$\iface$-spe\-cif\-ic BGP result addition} to~$\Omega$ for $\symBGP$ over~$\member$, denoted by $\bgpAdd{\Omega}{\symBGP}{\member}$, is
	a set of solution mappings that is defined as \removable{follows:}
	%a set of solution mappings that is defined as
	%the following set of solution mappings:
$\bgpAdd{\Omega}{\symBGP}{\member} \definedAs \Omega \Join \omega\bigl( \ifaceFct(\symBGP,\symRDFgraph) \bigr)$.
\end{mydefinition}

Finally, the following definition lifts the standard SPARQL algebra operators join and union into our algebra. In contrast to
	%our previous operators,
	$\xxxAlgebraOperatorName{tpAdd}$ and $\xxxAlgebraOperatorName{bgpAdd}$,
our $\xxxAlgebraOperatorName{join}$ operator captures the intention
	to obtain the two input sets of solution mappings independently and, then, join them only in
	%that the two input sets of solution mappings are obtained independently and, then, joined only by
the query federation engine alone.
	%\removable{G{\"{o}}rlitz and Staab's call this mediator joins~\cite{DBLP:series/sci/GorlitzS11,gorlitz2011splendid}.}
%
	Examples of
	%Specific
algorithms that can be used as implementations are a~(local) nested-loops
	%join~\cite{quilitz2008querying},
	join,
%
	%a group join~\cite{vidal2010efficiently},
a
	%simple
hash join~%
	%\cite{acosta2011anapsid,gorlitz2011splendid},
	\cite{acosta2011anapsid},
a symmetric hash join~\cite{acosta2011anapsid,saleem2018costfed}, or a~merge~join~\cite{charalambidis2015semagrow}.

\begin{mydefinition} \label{def:join&union}
Let $\Omega$ and $\Omega'$ be two sets of solution mappings.
%
The \definedTerm{join} of $\Omega$ and~$\Omega'$\!, denoted by $\join{\Omega}{\Omega'}$, is
	a set of solution mappings that is defined as \removable{follows:}
	%a set of solution mappings that is defined as
	%the following set of solution mappings:
$\join{\Omega}{\Omega'} \definedAs \Omega \cup \Omega' \!.$
%
The \definedTerm{union} of $\Omega$ and~$\Omega'$\!, denoted by $\union{\Omega}{\Omega'}$, is
	%a set of solution mappings that is defined as \removable{follows:}
	%a set of solution mappings that is defined as
	the following set of solution mappings:
$\union{\Omega}{\Omega'} \definedAs \Omega \cup \Omega' \!.$
\end{mydefinition}

\begin{myexample} \label{ex:union}
To represent the whole source assignment~$a'_\mathsf{ex}$~(cf.\ Example~\ref{ex:SourceAssignment:Syntax})
	%\removable{completely}
%
	\removable{as a logical plan}
we may combine the operators in Examples~\ref{ex:request} and~\ref{ex:tpAdd} with a $\xxxAlgebraOperatorName{union}$ operator as follows:
$\unionB{ \tpAdd{ \request{\symTP_2}{\member_2\!} }{\symTP_1}{\member_1\!} }{
\request{\lbrace\symTP_1,\symTP_2\rbrace\!}{\member_3}
} 
$.
\end{myexample}

	%Hereafter, we refer to every
	Hereafter, we call every
	%Every
expression that can be formed by using the operators defined in Definitions~\ref{def:request}--\ref{def:join&union}
	%as
	%is called
a \emph{HetFedA expression}. Note that each such expression defines a set of solution mappings and can be
	represented as an ordered~%
	%illustrated in the form of
	%illustrated as~a~%
tree.

% \begin{mydefinition} \label{def:HetFedA:Expression}
% 	%The notion of a
% 	A
% \definedTerm{HetFedA expression} is defined recursively as follows.
% \begin{enumerate}
% 	\item
% 		%Any symbol~$\Omega$ that denotes a set of solution mappings
% 		If $\Omega$ that denotes a set of solution mappings, then $\Omega$
% 	is a HetFedA expression.
% 
% 	\item If $\member = (\symRDFgraph,\iface)$ is a federation member with interface~$\iface = \ifaceTuple$ and $\ifaceReqLangExp$~is an expression in $\ifaceReqLang$, then $\request{\ifaceReqLangExp}{\member}$ is a HetFedA expression.
% 
% 	\item If
% 		%$\varphi$ is a HetFedA expression, $\symTP$ is a triple pattern, and $\member$ is federation member that supports triple pattern requests, then $\tpAdd{\varphi}{\symTP}{\member}$ is a HetFedA~expression.
% 		$\symTP$ is a triple pattern, and $\member$ is federation member that supports triple pattern requests, and $\varphi$ is a HetFedA expression, then so is $\tpAdd{\varphi}{\symTP}{\member}$.
% 
% 	\item If
% 		%$\varphi$ is a HetFedA expression, $\symBGP$ is a BGP, and $\member$ is federation member whose interface supports BGP requests, then $\bgpAdd{\varphi}{\symBGP}{\member}$ is a HetFedA~expression.
% 		$\symBGP$ is a BGP, and $\member$ is federation member whose interface supports BGP requests, and $\varphi$ is a HetFedA expression, then so is $\bgpAdd{\varphi}{\symBGP}{\member}$.
% 
% 	\item If
% 		%$\varphi_1$ and $\varphi_2$
% 		$\varphi_1, \varphi_2$
% 	are HetFedA expressions, then
% 		%$\join{\varphi_1}{\varphi_2}$ and $\union{\varphi_1}{\varphi_2}$ are HetFedA expressions.
% 		so are $\join{\varphi_1}{\varphi_2}$ and $\union{\varphi_1}{\varphi_2}$.
% \end{enumerate}
% \end{mydefinition}


\begin{myexample} \label{ex:HetFedA_expression}
The HetFedA expression in Example~\ref{ex:union} can be represented as the tree in Figure~\ref{fig:HetFedA_expression}(a), and it defines the same set of solution mappings as in~Example~\ref{ex:QuerySemantics}.
\end{myexample}

\begin{figure}[t]
    \centering
\scriptsize
% \small
%\footnotesize
    \begin{tabular}{c c c}
    \begin{forest}
for tree={s sep=0mm, inner sep=1mm, l=0}
        [$\xxxAlgebraOperatorName{union}$
         [$\xxxAlgebraOperatorName{tpAdd}^{\symTP_1}_{\member_1}$
          [$\xxxAlgebraOperatorName{req}^{\symTP_2}_{\member_2}$]
         ]
         [$\xxxAlgebraOperatorName{req}^{\lbrace\symTP_1,\symTP_2\rbrace\!}_{\member_3}$]
        ]
    \end{forest}
    &
    \begin{forest}
for tree={s sep=1mm, inner sep=1mm, l=0}
       [$\xxxAlgebraOperatorName{union}$
        [$\xxxAlgebraOperatorName{join}$
         [$\xxxAlgebraOperatorName{req}^{\symTP_1}_{\member_1\!}$]
         [$\xxxAlgebraOperatorName{req}^{\symTP_2}_{\member_2\!}$]
        ]
        [$\xxxAlgebraOperatorName{join}$
         [$\xxxAlgebraOperatorName{req}^{\symTP_1}_{\member_3\!}$]
         [$\xxxAlgebraOperatorName{req}^{\symTP_2}_{\member_3\!}$]
        ]
       ]
    \end{forest}
    &
    \begin{forest}
for tree={s sep=1mm, inner sep=1mm, l=0}
       [$\xxxAlgebraOperatorName{join}$
        [$\xxxAlgebraOperatorName{union}$
         [$\xxxAlgebraOperatorName{req}^{\symTP_1}_{\member_1\!}$]
         [$\xxxAlgebraOperatorName{req}^{\symTP_1}_{\member_3\!}$]
        ]
        [$\xxxAlgebraOperatorName{union}$
         [$\xxxAlgebraOperatorName{req}^{\symTP_2}_{\member_2\!}$]
         [$\xxxAlgebraOperatorName{req}^{\symTP_2}_{\member_3\!}$]
        ]
       ]
    \end{forest}
\\
    (a)
    &
    (b)
    &
    (c)
    \end{tabular}
	\caption{%
		%Tree representations of
		Trees representing
	HetFedA expressions that are logical plans for BGP~$\symBGP_\mathsf{ex}$ over federation~$\Fed_\mathsf{ex}$, created based on source assignments $a'_\mathsf{ex}$, (a) and (b), and $a_\mathsf{ex}$ (c)%
%~(cf.\ Example~\ref{ex:SourceAssignment:Syntax})%
	.}
	\label{fig:HetFedA_expression}
\end{figure}


% \todo{todo--Sijin}
% \inlinetodo{TODO: add an example of a HetFedA expression (and mention explicitly the set of solution mappings that it defines)}
% 
% Recall that source assignment $a_\mathsf{ex}$ in Example~\ref{ex:SourceAssignment:Syntax} is created based on $\symBGP_\mathsf{ex} = \lbrace \symTP_1, \symTP_2 \rbrace$ and $\Fed_\mathsf{ex} = \lbrace \member_1, \member_2 \rbrace$. Assume that each subquery is executed solely on given federation member, no intermediate results are used for other subqueries and no optimization on join order, a straighforward logical query plan can be represented as HetFedA expression:
% \begin{equation*}\label{ex:HetFedA expression_c}
% \begin{aligned}
% e = \join{\, \union{\, \request{\symTP_1}{\member_1} }{\,\request{\symTP_1}{\member_2} } }{\,\request{\symTP_2}{\member_1} }
% \end{aligned}
% \end{equation*}
% 
% %to update
% Rewrite for optimizing logical query:
% \begin{equation*}\label{ex:HetFedA expression_a}
% \begin{aligned}
% e = \tpAdd{\, \union{ \,\request{\symTP_1}{\member_1} }{  \,\request{\symTP_1}{\member_2} }}{\symTP_2}{\member_1}
% \end{aligned}
% \end{equation*}
% 
% \begin{equation*}\label{ex:HetFedA expression_b}
% \begin{aligned}
% e = \union{\, \tpAdd{\, \request{\symTP_2}{\member_1}  }{\symTP_1}{\member_1}  }{\, \tpAdd{\, \request{\symTP_2}{\member_1}  }{\symTP_1}{\member_2}  }
% \end{aligned}
% \end{equation*}
% 
% 
% Solution mappings are the same as $\mathsf{sols}(a)$~(cf.\ Example~\ref{ex:SourceAssignment:Semantics}).
% 
% Every HetFedA expression may be illustrated as a tree in which the operators are nodes and every operator that produces an input for another operator is a child of that other operator. 
% 
% \inlinetodo{TODO: add an example of such a tree // ACTUALLY, move this whole discussion of trees to Section6, because there may be cases in which we don't have a tree but just a rooted DAG}
% %to update
% \begin{figure}[htbp]
%     \centering
%     \begin{tabular}{c c c}
%     \begin{forest}
%         [join
%          [union
%           [$\request{\symTP_1}{\member_1}$
%           ]
%           [$\request{\symTP_1}{\member_2}$
%           ]
%          ]
%          [$\request{\symTP_2}{\member_1}$
%          ]
%         ]
%     \end{forest}
%     &
%     \begin{forest}
%         [$\tpAdd{}{\symTP_2}{\member_1}$
%          [union
%           [$\request{\symTP_1}{\member_1}$
%           ]
%           [$\request{\symTP_1}{\member_2}$
%           ]
%          ]
%         ]
%     \end{forest}
%     &
%     \begin{forest}
%         [union
%          [$\tpAdd{}{\symTP_1}{\member_1}$
%           [$\request{\symTP_2}{\member_1}$
%           ]
%          ]
%          [$\tpAdd{}{\symTP_1}{\member_2}$
%           [$\request{\symTP_2}{\member_1}$
%           ]
%          ]
%         ]
%     \end{forest}\\
%     (a)
%     &
%     (b)
%     &
%     (c)
%     \end{tabular}
% \end{figure}


With the following notion of an \emph{unoptimized plan} we introduce a generic approach to create an initial logical plan for any given source assignment%
	\removable{~(which may then be used as the starting point for logical query optimization)}%
.

\begin{mydefinition} \label{def:Translation2Plan:Unoptimized}
Let
	%$\Fed$ be a federation that is triple pattern accessible, let $\symBGP$ be a BGP, and let $a$ be a source assignment for~$\symBGP$ over~$\Fed$.
	$a$ be a source assignment for a BGP~$\symBGP$ over a triple pattern accessible federation~$\Fed$.
%
An \definedTerm{unoptimized plan} for $a$ is a HetFedA expression that is defined recursively as follows.
\begin{enumerate}

	\item If $a$ is of the form $\saBL \symBGP' \saBM \member \saBR$ where $\symBGP'\! = \lbrace \symTP_1, \symTP_2, ..., \symTP_n \rbrace$, then every HetFedA expression of the following form is an unoptimized plan for $a$:
	$$\joinB{ \,\joinB{ \ldots \,\joinB{ \,\joinB{ \request{\symTP_1}{\member} }{ \request{\symTP_2}{\member} } }{ \request{\symTP_3}{\member} } }{\ldots} }{ \request{\symTP_n}{\member} } .$$

	\item If $a$ is of the form $\saUL \, a_1 \oplus \cdots \oplus a_m \, \saUR$, then every HetFedA expression of the following form is an unoptimized plan for $a$:
	$$\union{ \,\union{ \ldots \,\union{ \,\union{\varphi_1}{\varphi_2} }{\varphi_3} }{\ldots} }{ \varphi_m } ,$$
	where, for every $i\in\lbrace 1,2,...,m\rbrace$,
		%\removable{subexpression~}%
	$\varphi_i$ is an unoptimized plan for $a_i$.

	\item If $a$ is of the form $\saJL \, a_1 \otimes \cdots \otimes a_k \, \saJR$, then every HetFedA expression of the following form is an unoptimized plan for $a$:
	$$\join{ \,\join{ \ldots \,\join{ \,\join{\varphi_1}{\varphi_2} }{\varphi_3} }{\ldots} }{ \varphi_n } ,$$
	where, for every $i\in\lbrace 1,2,...,m\rbrace$,
		%\removable{subexpression~}%
	$\varphi_i$ is an unoptimized plan for $a_i$.
\end{enumerate}
\end{mydefinition}

\begin{myexample} \label{ex:Translation2Plan:Unoptimized}
Figures~\ref{fig:HetFedA_expression}(b) and~%
	%\removable{Figures}%
~\ref{fig:HetFedA_expression}(c) illustrate tree representations of unoptimized plans for
	%our example
	the
source assignments~$a'_\mathsf{ex}$ and~$a_\mathsf{ex}$~(cf.\ Example~\ref{ex:SourceAssignment:Syntax}), respectively.
\end{myexample}

It can be shown that every unoptimized plan produces the correct query result as long as it has been constructed based on a correct source~assignment.

% This proposition follows from Definitions~\ref{def:QuerySemantics}, \ref{def:SourceAssignment:Semantics},
% \ref{def:CorrectSourceAssignment},
% and
% 	%\ref{def:request}--\ref{def:join&union}
% \ref{def:request}--\ref{def:Translation2Plan:Unoptimized}.

% \inlinetodo{TODO: move the previous definition to the next section (about algebra programs) and define the notion of an unoptimized plan to be a program (rather than and expression) where this program consists only of one expression, namely the one given in the definition above.}

\begin{myproposition} \label{thm:Translation2Plan:Unoptimized}
Let
	%$\Fed$ be a federation that is triple pattern accessible, let $\symBGP$ be a BGP, and let $a$ be a source assignment for~$\symBGP$ over~$\Fed$.
	$a$ be a source assignment for a BGP~$\symBGP$ over a triple pattern accessible federation~$\Fed$,
and $\Omega$ be the set of solution mappings defined by an unoptimized plan for $a$.
If $a$ is correct, it holds that $\eval{\symBGP}{\Fed} = \Omega$.
\end{myproposition}

% \begin{proof}
% See Definitions~\ref{def:QuerySemantics}, \ref{def:SourceAssignment:Semantics}, \ref{def:CorrectSourceAssignment}, \ref{def:request}--\ref{def:Translation2Plan:Unoptimized}, in combination with definitions in Section~\ref{sec:Preliminaries}.
% \end{proof}

\begin{proof}
	\removable{Proposition~\ref{thm:Translation2Plan:Unoptimized} follows readily} from Definitions~\ref{def:QuerySemantics}, \ref{def:SourceAssignment:Semantics},
\ref{def:CorrectSourceAssignment},
% \removable{and}
	%\ref{def:request}--\ref{def:join&union}
\ref{def:request}--\ref{def:Translation2Plan:Unoptimized}, combined with \removable{the definition of the SPARQL algebra and
	%evaluation function $\eval{\symPattern}{\symRDFgraph}$%
	of evaluation $\eval{\symPattern}{\symRDFgraph}$%
}%
	~(cf.\ Section~\ref{sec:Preliminaries})%
	%~(Section~\ref{sec:Preliminaries})%
.
\end{proof}


% \inlinetodo{Physical operators that can be used to implement our logical operator:
% tpAdd:\\
% 1. form of index nested-loop join: for every binding in the outer relation, scan the inner relation and add the bindings that match the join condition to the result set\\
% * DARQ ``bind join'' \cite{quilitz2008querying}, njoin\cite{vidal2010efficiently}\\
% %
% 2. bind join (also in NLJ fashion): the intermediate results from outer relations are passed to the inner relations. (send sub-query for the inner relation, implemented using SPARQL FILTER or VALUES expression)\\
% * CostFed\cite{saleem2018costfed}, SemaGrow\cite{charalambidis2015semagrow}, Splendid\cite{gorlitz2011splendid}
% %
% 3. bound join (improved bind join): group a set of mappings in a single query using UNION expression (bind join requires a subquery for each mapping)\\
% * SemaGrow\cite{charalambidis2015semagrow}, FedX\cite{schwarte2011fedx}, Lusail\cite{abdelaziz2017lusail}\\
% %
% 4. distributed semi-join: buffer the obtained variable binding set and sends them in a batch as condition in a SPARQL FILTER expression, appended to the wrapped triple pattern to a remote SPARQL endpoint\\
% * distributed semi-join paper\cite{zemanek2008optimizing}\\
% %
% \textbf{bgpAdd} (not sure):\\
% 1. bind join\\
% 2. bound join\\
% 3. distributed semi-join
% \\
% \textbf{join:}
% \\
% 1. naive (server-side) nested-loop join: for every binding in the outer relation, scan the inner relation and add the bindings that match the join condition to the result set\\
% * DARQ ``nested join'' \cite{quilitz2008querying},
% \\
% 1. group join(gjoin)\cite{vidal2010efficiently}: independently evaluates star-shaped groups, matches their results
% \\
% 2. symmetric hash join: \\
% * ANAPSID\cite{acosta2011anapsid}: (adaptive group join (agjoin) and adaptive Dependent Join(adjoin))
% maintain a hash table for the data retrieved from sources A and B.\\
% * CostFed\cite{saleem2018costfed}\\
% %
% 3. traditional hash join\\
% SPLENDID~\cite{gorlitz2011splendid}
% ANAPSID\cite{acosta2011anapsid}(used for comparison)
% \\
% 4. Merge join: requests for its input to be sorted on the join variables\\
% * SemaGrow\cite{charalambidis2015semagrow}
% }


==> programs.tex <==
\subsection{Algebra Programs} \label{ssec:AlgebraPrograms}

	%This section introduces
	We now introduce
a notion of programs that are built by combining HetFedA~expressions and that
	%can
capture options for interoperator parallelism and reuse of intermediate results.
%
As a motivation, consider the following HetFedA expression.
\begin{equation} \label{eq:AlgebraPrograms:MotivatingExampleExpression}
\unionB{
	\;
	\tpAdd{ \request{\symTP_1}{\member_1\!} }{\symTP_2}{\member_2\!}
	\;
 }{
	\;
	\tpAdd{ \request{\symTP_1}{\member_1\!} }{\symTP_2}{\member_3\!}
	\;
}
\end{equation}

Notice that this expression contains the subexpression $\request{\symTP_1}{\member_1\!}$ twice. If we let $\Omega^*\!$ denote the set of solution mappings that this subexpression defines, i.e.,
	%\begin{equation} \label{eq:AlgebraPrograms:MotivatingExampleSubexpression} \Omega^*\! = \request{\symTP_1}{\member_1\!}	, \end{equation}
	$\Omega^*\! = \request{\symTP_1}{\member_1\!}$,
then the following HetFedA expression defines the same
	set of solution mappings
	%query result
as the one in equation~(\ref{eq:AlgebraPrograms:MotivatingExampleExpression}) above. 
\begin{equation} \label{eq:AlgebraPrograms:MotivatingExampleExpression2}
\unionB{
	\;
	\tpAdd{ \Omega^* }{\symTP_2}{\member_2\!}
	\;
 }{
	\;
	\tpAdd{ \Omega^* }{\symTP_2}{\member_3\!}
	\;
}
\end{equation}

	This syntactic difference between the two expressions can be used as a way to distinguish two different approaches to produce the set of solution mappings that they define:
	%For our notion of HetFedA programs/plans we interpret the two expressions differently:
%
By
	breaking
	%splitting
the subexpression
	%in~(\ref{eq:AlgebraPrograms:MotivatingExampleSubexpression})
	$\request{\symTP_1}{\member_1\!}$
out of the expression in equation~(\ref{eq:AlgebraPrograms:MotivatingExampleExpression2}), we capture the intention
	to produce the result of the subexpression only once and, then, feed it
	%that the subexpression is evaluated only once and its result is fed
	%to execute the subexpression only once and its result is fed
into the two $\xxxAlgebraOperatorName{tpAdd}$ operators. In contrast,
	the fact that, in the first case, the subexpression is inlined directly into the expression~(\ref{eq:AlgebraPrograms:MotivatingExampleExpression}) indicates that the result of the subexpression is meant to be produced twice in two separate processes\hidden{, namely once as input for the first $\xxxAlgebraOperatorName{tpAdd}$ operator and once more as input for the second $\xxxAlgebraOperatorName{tpAdd}$ operator}.
	%for a HetFedA expression that contains the same subexpression multiple times, as is the case in equation~(\ref{eq:AlgebraPrograms:MotivatingExampleExpression}), we define that such an expression captures the intention that each occurrence of a subexpression results in/induces/leads to a separate evaluation of that subexpression .

In general, for the following notion of HetFedA programs, we define that each HetFedA expression captures the intention that each occurrence of a subexpression within the HetFedA expression results in/induces/leads to
	%a separate evaluation of that subexpression.
	a ``separate'' process to produce the result of the subexpression.

\inlinetodo{... TODO ...}

\begin{mydefinition} \label{def:HetFedA:Program}
A \definedTerm{HetFedA program} is a tuple~$(\mathbf{\Omega},\mathbf{\Phi},\psi,\Omega_\mathsf{R})$ where
\begin{itemize}
	\item $\mathbf{\Omega}$ is a finite set of symbols that each denotes a set of solution mappings,
	\item $\mathbf{\Phi}$ is a finite set of HetFedA expressions such that $|\mathbf{\Omega}| = |\mathbf{\Phi}|$,
	\item $\psi$ is a bijection $\psi \!: \mathbf{\Omega} \rightarrow \mathbf{\Phi}$, and
	\item $\Omega_\mathsf{R} \in \mathbf{\Omega}$.
\end{itemize}
\end{mydefinition}

\begin{mydefinition} \label{def:HetFedA:GroundedProgram}
A HetFedA program~$(\mathbf{\Omega},\mathbf{\Phi},\psi,\Omega_\mathsf{R})$ is \definedTerm{grounded} if for every $\varphi \in \mathbf{\Phi}$ and every subexpression $\Omega$ of $\varphi$ such that $\Omega$ is a symbol denoting a set of solution mappings, it holds that $\Omega \in \mathbf{\Omega}$.
\end{mydefinition}

\begin{mydefinition} \label{def:HetFedA:AcyclicProgram}
A grounded HetFedA program~$(\mathbf{\Omega},\mathbf{\Phi},\psi,\Omega_\mathsf{R})$ is \definedTerm{acyclic} if $\Omega_\mathsf{R}$ is not a subexpression of%
	\removable{\ the HetFedA expression}%
~$\psi(\Omega_\mathsf{R})$
and either $|\mathbf{\Omega}| = 1$
or there exists an acyclic HetFedA program~$(\mathbf{\Omega}',\mathbf{\Phi}',\psi',\Omega_\mathsf{R}')$ such that the following three properties hold:
\begin{enumerate}
	\item $\Omega_\mathsf{R} \notin \mathbf{\Omega}'$,
	\item $\mathbf{\Omega} = \mathbf{\Omega}' \cup \lbrace \Omega_\mathsf{R} \rbrace$, and
	\item $\psi(\Omega)=\psi'(\Omega)$ for all $\Omega \notin \mathbf{\Omega}'$.
\end{enumerate}
\end{mydefinition}

\inlinetodo{... TODO ...}

\begin{myexample}
\begin{align*}
e &= \join{ e_1 }{ e_1 }
\\
%E = \lbrace (v,e_1) \rbrace \text{ where }
e_1 &= \request{\symBGP_2}{\member_2}
\end{align*}
---------
\begin{align*}
e &= \join{\request{\symBGP_2}{\member_2}}{\request{\symBGP_2}{\member_2}}
\\
E = \emptyset
\end{align*}

\end{myexample}



Every expression that can be formed by using the operators defined in Definitions~\ref{def:request}--\ref{def:join&union} is called a \emph{HetFedA expression}. Note that each such expression defines a set of solution mappings. Based on the source assignment of SemaGrow in the table~\ref{tb:source-assignment-examples}, the query execution plan for basic graph pattern B over the federation F can be expressed as HetFedA expression in the following:
\begin{equation*}
\begin{aligned}
e &= \union{\, \tpAdd{\, \tpAdd{\,\union{ \, \tpAdd{ \, \request{\symBGP_1}{\member_1} \,}{\symTP_4}{\member_2} \, }{\, \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \tpAdd{ \,\request{\symBGP_1}{\member_1} \,}{\symTP_4}{\member_4} \, } \,}{\symTP_3}{\member_2} \,}{\symTP_5}{\member_2} \,}{\, \\
&\quad \quad \quad \quad \tpAdd{\, \tpAdd{ \, \union{\, \tpAdd{\, \request{\symBGP_1}{\member_1} \,}{\symTP_4}{\member_2} \, }{ \, \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \tpAdd{\, \request{\symBGP_1}{\member_1} \, }{\symTP_4}{\member_4}\, } \, }{\symTP_3}{\member_2}\, }{\symTP_5}{\member_4} \, \\
&\quad \quad \quad \quad }
\end{aligned}
\end{equation*}

The HetFedA program is $(e,E)$:

\begin{equation*}
\begin{aligned}
e &= \union{v_1}{v_2} \\
E &= \lbrace (v_1,e_1)\, (v_2, e_2)\,(v_3,e_3) \, (v_4,e_4)\, (v_5,e_5)\, (v_6, e_6)\, (v_7,e_7) \rbrace \\
& \text{ where } \\
& \quad e_1 = \tpAdd{v_3}{\symTP_5}{\member_2}, \quad e_2 = \tpAdd{v_3}{\symTP_5}{\member_4} \\
& \quad e_3 = \tpAdd{v_4}{\symTP_3}{\member_2}, \quad e_4 = \union{v_5}{v_6} \\
& \quad e_5 = \tpAdd{v_7}{\symTP_4}{\member_2}, \quad e_6 = \tpAdd{v_7}{\symTP_4}{\member_4} \\
& \quad e_7 = \request{\symBGP_1}{\member_1}
\end{aligned}
\end{equation*}

According to the definition~\ref{def:QuerySemantics}, the evaluation of a SPARQL graph pattern~$\symPattern$ over a federation~$\Fed$ is denotes as
$\eval{\symPattern}{\Fed}$. The set of solution mappings of this specific expression defined is as follows:

\todo[inline]{solution mappging}
%$$\eval{\symPattern}{\Fed} = \union{\eval{\symPattern_1}{DrugBank}}{\eval{\symPattern_2}{KEGG}}$$

$\symBGP = \{ \symTP_1, ..., \symTP_5 \}$ \\
$\eval{\symBGP}{\Fed} = \eval{ \symBGP }{\symRDFgraph_\mathrm{union}}$ \\
$\eval{ \symBGP }{\symRDFgraph_\mathrm{union}} = \eval{\symTP_1 \OpAND\ ... \OpAND\ \symTP_5 }{\symRDFgraph_\mathrm{union}}$ \\
$\eval{\symTP_1 \OpAND\ ... \OpAND\ \symTP_5 }{\symRDFgraph_\mathrm{union}} = \eval{\symTP_1}{\symRDFgraph_\mathrm{union}} \Join \eval{\symTP_2}{\symRDFgraph_\mathrm{union}} \Join ...  \Join  \eval{\symTP_5}{\symRDFgraph_\mathrm{union}}$

Every HetFedA expression may be illustrated as a tree in which the operators are nodes and every operator that produces an input for another operator is a child of that other operator. 
\begin{figure}[htbp]
  \centering
  \begin{tabular}{p{0.62\textwidth} p{0.3\textwidth} }
    \begin{forest}
        [union
         [$\tpAdd{}{\symTP_5}{\member_2}$
           [$\tpAdd{}{\symTP_3}{\member_2}$
            [union
             [$\tpAdd{}{\symTP_4}{\member_2}$
              [$\request{\symBGP_1}{\member_1}$]
             ]
             [$\tpAdd{}{\symTP_4}{\member_4}$
              [$\request{\symBGP_1}{\member_1}$]
             ]
            ]
           ]
         ]
         [$\tpAdd{}{\symTP_5}{\member_4}$
           [$\tpAdd{}{\symTP_3}{\member_2}$
            [union
             [$\tpAdd{}{\symTP_4}{\member_2}$
              [$\request{\symBGP_1}{\member_1}$]
             ]
             [$\tpAdd{}{\symTP_4}{\member_4}$
              [$\request{\symBGP_1}{\member_1}$]
             ]
            ]
           ]
         ]
        ]
    \end{forest}
    &
    \begin{forest}
        [union
         [$\tpAdd{}{\symTP_5}{\member_2}$
           [$\tpAdd{}{\symTP_3}{\member_2}$, name = B
            [union
             [$\tpAdd{}{\symTP_4}{\member_2}$
              [$\request{\symBGP_1}{\member_1}$], name = D
             ]
             [$\tpAdd{}{\symTP_4}{\member_4}$, name = C
              [, no edge]
             ]
            ]
           ]
         ]
         [$\tpAdd{}{\symTP_5}{\member_4}$, name = A
           [, no edge
            [, no edge
             [, no edge
              [, no edge]
             ]
             [, no edge
              [, no edge]
             ]
            ]
           ]
         ]
        ]
    \draw (B) -- (A);
    %\draw (C) -- (D);
    \end{forest}
  \end{tabular}
  \caption{Tree-type expression. Left:XXXX. Right:XXXXX} 
  \label{}
\end{figure}

\todo[inline]{discuss parallelism}
